The Maximum Cardinality Cut Problem is Polynomial in Proper Interval Graphs

It is known that the maximum cardinality cut problem is NP-hard even in chordal graphs. In this paper, we consider the time complexity of the problem in proper interval graphs, a subclass of chordal graphs, and propose a dynamic programming algorithm which runs in polynomial-time.

==> intro.tex <==
A \emph{cut} of a graph $G=(V(G),E(G))$ is a partition of $V(G)$ into two subsets $S, \bar{S}$ where $\bar S=V(G)\setminus S$. The \emph{cut-set} of $(S,\bar{S})$ is the set of edges of $G$ with exactly one endpoint in $S$. The maximum cardinality cut problem ($\maxcut$) is to find a cut with a maximum size cut-set, of a given graph.

$\maxcut$ remains $\nph$ when restricted to the following graph classes: chordal graphs, undirected path graphs, split graphs, tripartite graphs, co-bipartite graphs \cite{Bodlaender00onthe}, unit disk graphs \cite{DK2007} and total graphs \cite{Guruswami1999217}. On the other hand, it was shown that $\maxcut$ can be solved in polynomial-time in planar graphs \cite{hadlock1975finding}, in line graphs \cite{Guruswami1999217}, and the class of graphs factorable to bounded treewidth graphs \cite{Bodlaender00onthe}.

Proper interval graphs are not necessarily planar. They are not necessarily line graphs either, since the graph $\bar{A}$ consisting of 6 vertices is a proper interval graph, but a forbidden subgraph of line graphs \cite{Beineke1970129}. In \cite{BES15-MaxCut-JOCOSpecialIssue}, we have shown that co-bipartite chain graphs are not factorable to bounded treewidth graphs. Since co-bipartite chain graph are proper interval graphs, this result holds for them too. Therefore, the above mentioned results do not imply a polynomial-time algorithm for proper interval graphs.

Despite the existence of polynomial-time algorithms for some subclasses of proper interval graphs (split indifference graphs \cite{Bodlaender2004} and co-bipartite chain graphs \cite{BES15-MaxCut-JOCOSpecialIssue}), the complexity of $\maxcut$ in proper interval graphs was open. In this work, we generalize the dynamic programming algorithm in \cite{BES15-MaxCut-JOCOSpecialIssue} to proper interval graphs using the bubble model of proper interval graphs introduced in \cite{HMP09}.

